Dynamic self-triggered control for nonlinear systems based on hybrid Lyapunov functions

Self-triggered control (STC) is a well-established technique to reduce the amount of samples for sampled-data systems, and is hence particularly useful for Networked Control Systems. At each sampling instant, an STC mechanism determines not only an updated control input but also when the next sample should be taken. In this paper, a dynamic STC mechanism for nonlinear systems is proposed. The mechanism incorporates a dynamic variable for determining the next sampling instant. Such a dynamic variable for the trigger decision has been proven to be a powerful tool for increasing sampling intervals in the closely related concept of event-triggered control, but was so far not exploited for STC. This gap is closed in this paper. For the proposed mechanism, the dynamic variable is chosen to be the filtered values of the Lyapunov function at past sampling instants. The next sampling instant is, based on the dynamic variable and on hybrid Lyapunov function techniques, chosen such that an average decrease of the Lyapunov function is ensured. The proposed mechanism is illustrated with a numerical example from the literature. For this example, the obtained sampling intervals are significantly larger than for existing static STC mechanisms. This paper is the accepted version of [1], containing also proofs of the main results.

==> proof_theo2.tex <==
% !TeX root = stc.tex
%\begin{proof}
\subsection{Proof of Theorem~\ref{theo_stab2}}
\label{appendix_2}
		This proof follows the same lines as the proof of Theorem~\ref{theo_stab}. Therefore, we describe here only the differences to  this proof. Using similar arguments as in the proof of Theorem~\ref{theo_stab}, we observe that $\svar_{j+1} -\svar_j \geq t_{\min}$ holds and that
		\begin{equation}
			\label{eq_V_bound_theo2}
			V(x(\tvar_{j+1})) \leq e^{-\tilde{\epsilon} (\svar_{j+1} - \svar_j)} \max \left\lbrace V(x(\tvar_j),\eta(\tvar_j) \right\rbrace,
		\end{equation}
		where $\tilde \epsilon = \min \left\lbrace \epsilon_1,\epsilon_\refer \right\rbrace$. Due to the choice of $S(\eta,x)$ in \eqref{eq_S_ref} and $\svar_{j+1}-\svar_j = \Gamma(x(\tvar_j),\eta(\tvar_j))$, we know that
		\begin{equation}
		\label{eq_eta_bound_theo2}
			\eta(\tvar_j) = e^{-\epsilon_\refer\svar_j} \eta(\tvar_0)
		\end{equation}  holds for all $j \in \mathbb{N}_0$. Now suppose that 
		\begin{equation}
		\label{eq_ia_theo2}
			V(x(\tvar_j)) \leq e^{-\tilde \epsilon \svar_{j} } \max \left \lbrace V(x(\tvar_0)), \eta(\tvar_0) \right\rbrace.
		\end{equation} Then it follows from \eqref{eq_V_bound_theo2} and \eqref{eq_eta_bound_theo2} with $\epsilon_\refer \geq \tilde\epsilon$ that 
%		\begin{equation*}
			$V(x(\tvar_{j+1})) \leq e^{-\tilde \epsilon \svar_{j+1} } \max \left \lbrace V(x(\tvar_0)), \eta(\tvar_0) \right\rbrace$.
%		\end{equation*}
		Since \eqref{eq_ia_theo2} holds for $j = 0$, we can thus conclude by induction that it holds for all $j\in\mathbb{N}_0$ and thus that 
		\begin{align*}
			&V(x(\tvar_{j+1}))\\  \leq& e^{-\tilde \epsilon \svar_{j} }  \max \left \lbrace \bar{\alpha}_V\left(\norm{x(\tvar_0)}\right), \eta(\tvar_0) \right\rbrace\\
			 \leq& e^{-\tilde \epsilon \left(\frac{\svar_{j}+jt_{\min}}{2}\right)}  \max \left \lbrace \bar{\alpha}_V\left(\norm{\begin{bmatrix}
			 x(\tvar_0)\\
			 \eta(\tvar_0)
			 	\end{bmatrix}}\right), \norm{\begin{bmatrix}
			 	x(\tvar_0)\\
			 	\eta(\tvar_0)
			 	\end{bmatrix}} \right\rbrace\\
			 \eqqcolon & \tilde{\beta}_1\left(\norm{\begin{bmatrix}
			 		x(\tvar_0)\\
			 		\eta(\tvar_0)
			 		\end{bmatrix}},\svar_j,j\right).
		\end{align*}
%		Here, $t_{\max}$ is chosen as in the proof of Theorem~\ref{theo_stab}. 
		Note that $\tilde{\beta}_1$ is a class $\mathcal{K}\mathcal{L}\mathcal{L}$ function.
		The remainder of this proof is similar as the remainder of the proof of Theorem~\ref{theo_stab} after \eqref{eq_Vk_bound_theo2} and thus omitted. \hfill\hfill\qed
%	\end{proof}

==> proof_theo3.tex <==
% !TeX root = stc.tex
%	\begin{proof}
\subsection{Proof of Theorem~\ref{theo_stab3}}
\label{appendix_3}
		This proof follows the same lines as the proof of Theorem~\ref{theo_stab}. Therefore, we describe here only the differences to  this proof. Using similar arguments as in the proof of Theorem~\ref{theo_stab}, we observe that $\svar_{j+1} -\svar_j \geq t_{\min}$ holds and that
		\begin{equation}
		\label{eq_V_bound_theo3}
		V(x(\tvar_{j+1})) \leq e^{-\tilde{\epsilon} (\svar_{j+1} - \svar_j)} \max \left\lbrace V(x(\tvar_j),\eta(\tvar_j) \right\rbrace,
		\end{equation}
		where $\tilde \epsilon = \min \left\lbrace \epsilon_1,\epsilon_\refer \right\rbrace$. Moreover, due to the choice of $S(\eta,x)$ in \eqref{eq_S_iir}, we know that
%		\begin{align}
%		\label{eq_eta_bound_theo3}
		$\eta(\tvar_{j+1})  \leq (\hat{r}+\tilde{r}) \max \left\lbrace V(x(\tvar_j),\eta(\tvar_j)) \right\rbrace$
%		\end{align}  
		 for all $k \in \mathbb{N}_0$. We can thus infer  for $\rho = \max \left\lbrace \hat{r}+\tilde{r} , e^{-\tilde{\epsilon} t_{\min}}\right\rbrace <1$ from \eqref{eq_V_bound_theo3} that
%		that 
		\begin{equation*}
%		\label{eq_max_dec_theo3}
			\max \left\lbrace \eta(\tvar_{j+1}), V(x(\tvar_{j+1})) \right\rbrace \leq \rho \max \left\lbrace \eta(\tvar_j), V(x(\tvar_j)) \right\rbrace.
		\end{equation*}
	  Using
%		 \eqref{eq_max_dec_theo3}
		this recursively, we obtain 
		\begin{align}
			\nonumber &\max \left\lbrace \eta(\tvar_{j}), V(x(\tvar_{j})) \right\rbrace \\
			\nonumber \leq& \rho^j  \max \left\lbrace \eta(\tvar_0), V(x(\tvar_0)) \right\rbrace\\
			\nonumber\leq& \rho^{\frac{j}{2} + \frac{\svar_j}{2\svar_{\max}}} \max\left\lbrace \eta(\tvar_0),\bar{\alpha}_V\left(\norm{x(\tvar_0)}\right) \right\rbrace\\
%			\nonumber\leq& \rho^{\frac{j}{2} + \frac{\svar_j}{2\svar_{\max}}} \max\left\lbrace \norm{\begin{bmatrix}
%				\eta(\tvar_0)\\
%				x(\tvar_0)
%				\end{bmatrix}},\underline{\alpha}_V\left(\norm{\begin{bmatrix}
%				\eta(\tvar_0)\\
%				x(\tvar_0)
%				\end{bmatrix}}\right) \right\rbrace\\
			\nonumber\eqqcolon& \tilde{\beta}_1\left(\norm{\begin{bmatrix}
				\eta(\tvar_0)\\
				x(\tvar_0)
				\end{bmatrix}},\svar_j,j\right).
		\end{align}
				with $t_{\max}$ as in the proof of Theorem~\ref{theo_stab}. Note that $\tilde{\beta}_1$ is a class $\mathcal{K}\mathcal{L}\mathcal{L}$ function that bounds $V(x(\tvar_j))$ and $\eta(\tvar_j)$.
				The remainder of this proof is similar as the remainder of the proof of Theorem~\ref{theo_stab} after \eqref{eq_eta_bound_k} and thus omitted. \hfill\hfill\qed
%	\end{proof}
